Disentangled 3D Scene Generation with Layout Learning

We introduce a method to generate 3D scenes that are disentangled into their component objects. This disentanglement is unsupervised, relying only on the knowledge of a large pretrained text-to-image model. Our key insight is that objects can be discovered by finding parts of a 3D scene that, when rearranged spatially, still produce valid configurations of the same scene. Concretely, our method jointly optimizes multiple NeRFs from scratch - each representing its own object - along with a set of layouts that composite these objects into scenes. We then encourage these composited scenes to be in-distribution according to the image generator. We show that despite its simplicity, our approach successfully generates 3D scenes decomposed into individual objects, enabling new capabilities in text-to-3D content creation. For results and an interactive demo, see our project page at https://dave.ml/layoutlearning/

==> tables/01_ablation.tex <==
\setlength{\tabcolsep}{0.3em} %
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\multirow{3}{*}{Method} & \multicolumn{4}{c}{Average Score $\uparrow$}      \\
  & \multicolumn{2}{c}{CLIP B/16} & \multicolumn{2}{c}{CLIP L/14} \\
  & Color          & Geo          & Color          & Geo                 \\ \midrule
\textcolor{gray}{Random objects} &     \textcolor{gray}{23.4}   & \textcolor{gray}{22.4}  & \textcolor{gray}{17.2}    & \textcolor{gray}{18.3}  \\
\textcolor{gray}{Per-object SDS}        &  \textcolor{gray}{32.3}  &  \textcolor{gray}{30.5} & \textcolor{gray}{27.2} & \textcolor{gray}{25.9}  \\   \midrule
$K$ NeRFs   & 26.7    & 25.4  & 21.0    & 21.2  \\
+ Per-NeRF losses & 27.3 & 26.1 & 21.6 & 22.6 \\
+ Empty NeRF loss  & 27.7 & 26.2 & 22.8 & 23.2  \\ 
+ Learn layout  & 29.9 & 28.8 & 24.9& 23.5 \\
+ Learn $N$ layouts  &   \textbf{31.3} & \textbf{29.9} & \textbf{27.1} & \textbf{24.8} \\ \midrule
Relative layouts  & 30.4    & 29.2  &   25.7  & 24.0  \\
View dep. prompt & 31.0    & 29.1  &  25.6   & 23.6  \\ \bottomrule
\end{tabular}
}



 

